NNQS-Transformer: an Efficient and Scalable Neural Network Quantum States Approach for Ab initio Quantum Chemistry

Neural network quantum state (NNQS) has emerged as a promising candidate for quantum many-body problems, but its practical applications are often hindered by the high cost of sampling and local energy calculation. We develop a high-performance NNQS method for \textit{ab initio} electronic structure calculations. The major innovations include: (1) A transformer based architecture as the quantum wave function ansatz; (2) A data-centric parallelization scheme for the variational Monte Carlo (VMC) algorithm which preserves data locality and well adapts for different computing architectures; (3) A parallel batch sampling strategy which reduces the sampling cost and achieves good load balance; (4) A parallel local energy evaluation scheme which is both memory and computationally efficient; (5) Study of real chemical systems demonstrates both the superior accuracy of our method compared to state-of-the-art and the strong and weak scalability for large molecular systems with up to $120$ spin orbitals.

==> Makefile <==
base_name := Manuscript
datestamp := $(shell date +"%Y-%m-%d")
workdir   := $(shell basename $(shell pwd))


%.pdf: %.tex
	pdflatex --interaction=nonstopmode $<
	bibtex $*.aux
	pdflatex --interaction=nonstopmode $<
	pdflatex --interaction=nonstopmode $<


all: $(base_name).pdf  
	(evince $(base_name).pdf  &)


$(base_name).pdf: $(base_name).tex $(base_name).bib 

figures:
	$(MAKE) -C figures

dated:
	[ ! -d archive ] && mkdir archive
	$(MAKE) pdf
	cp -a $(base_name).pdf archive/$(base_name)-$(datestamp).pdf

tgz:
	$(MAKE) clean
	cd .. && tar -zcvf $(base_name)-$(datestamp).tgz $(workdir)

backup:
	$(MAKE) tgz
	cd .. && rsync -avizP $(base_name)-$(datestamp).tgz barin:backup/.

semiclean:
	rm -f *~ *.aux *.bbl *.blg *.brf *.bmt *.dvi *.log *.toc \
	$(base_name).pdf $(base_name).ps $(base_name).out $(base_name)Notes.bib

figuresclean:
	$(MAKE) -C figures clean

clean:
	$(MAKE) semiclean

.PHONY: clean figuresclean semiclean backup


==> algo.tex <==
\begin{algorithm}
\LinesNumbered
\label{alg:preprocess}
\KwIn{pauliStrings, n\_qubits}
\KwResult{idxs, pmXY\_buf, pmYZ\_buf, coeffs\_buf}
% \BlankLine

{$N, K \gets n\_qubits, \text{length(pauliStrings)}$\\}
$pmXY, pmYZ \gets \text{zeros}(N,K), \text{zeros}(N,K)$\\

\For{$(i, (coeff, pauliStr))$ \textbf{in} \text{enumerate(pauliStrings)}}{
    $Y_{occ} \gets 0$ \tcp{occurrence for Y}
    \tcc{Construct Pauli mat XY and Pauli mat YZ}
    \For{$(p, pauli)$ \textbf{in} pauliStr}{
        \If{$pauli == "X"$}{
            $pmXY[p, i] \gets 1$\\
        }
        \ElseIf{$pauli == "Y"$}{
            $pmXY[p, i] \gets pmYZ[p, i] \gets 1$\\
            $Y_{occ} \gets Y_{occ} + 1$\\
        }
        \Else{$pmYZ[p, i] \gets 1$}
    }
    \tcc{New coefficients: fuse const calculation}
    $coeff \gets \text{real}(coeff) \times \text{real}((-i)^{Y_{occ}})$ \\

    \tcc{Compressed Pauli mat XY using Dict}
    $sid = \_encode2id(pmXY[:,i])$\\
    \If{\textbf{not} \text{haskey(coeffs\_dict, sid)}}{
        $pmXY\_dict[sid] \gets pmXY[:,i]$\\
    }
    $coeffs\_dict[sid].\text{append}(coeff)$\\
    $pmYZ\_dict[sid].\text{append}([pmYZ[:,i]])$\\
}

\tcc{Compacting data into new continuous buffer}
$L \gets pmXY\_dict.count; idx \gets 0$\\
% $pmXY\_buf, pmYZ\_buf, coeffs\_buf, idxs, idx \gets$ \newline $\text{zeros(N, L)}, \text{zeros(N, K)}, \text{zeros(K)}, \text{zeros(L+1)}, 0$\\

\For{$(i, (sid, pm23))$ \textbf{in} \text{enumerate}(pmYZ\_dict)}{
    $num \gets \text{length}(pm23)$\\
    $pmYZ\_buf[:,idx:idx+num] \gets pm23$ \\
    $pmXY\_buf[:, i] \gets pmXY\_dict[sid]$\\
    $coeffs\_buf[idx:idx+num] \gets coeffs\_dict[sid]$ \\
    $ idx \gets idx + num$; $idxs[i] \gets idx$\\
}

% \Return{$idxs, pmXY\_buf, pmYZ\_buf, coeffs\_buf$}
% \end{algorithmic}
\caption{Preprocess: Hamiltonian data structure optimizations}
\end{algorithm}




\begin{algorithm}
\LinesNumbered
\caption{Calculate Local Energy}
\label{alg:calculate_local_energy}
\KwIn{$\text{idxs}$, $\text{pmXY}$, $\text{pmYZ}$, $\text{coeffs}$, $\text{states}$}

$\text{eloc} \leftarrow 0.0$\\
\For{$\text{state}$ \textbf{in} $\text{states}$}{
    \For{$i \leftarrow 0$ \KwTo $\text{size(pmXY, 2)}$}{
      \tcc{calculate coupled coef}
      $\text{coef} \leftarrow 0.0$\\
      \For{$j \leftarrow \text{idxs}[i]$ \KwTo $\text{idxs}[i+1]$}{
        $\text{tstate} \leftarrow \text{pmYZ}[:, j] \& \text{state}$\\
        $\text{coef} \leftarrow \text{coef} + ((-1)^{\text{cnt\_1}(\text{tstate})}) \times \text{coeffs}[j]$\\
      }
      $\text{cpld\_coefs}[i] \leftarrow \text{coef}$\\
    
      \tcc{calculate coupled states}
      $\text{cpld\_states}[:, i] \leftarrow \text{xor}(\text{state}, \text{pmXY}[:, i])$\\
    }

    \tcc{accumulate local energy of the state}
    $\text{eloc} += \text{dot}(\Psi(\text{cpld\_states}), \text{cpld\_coefs}) / \Psi(\text{state})$\\
}
\KwRet{$\text{eloc}$}\\
\end{algorithm}


\begin{algorithm}
\DontPrintSemicolon
\LinesNumbered
\SetAlgoLined
\KwIn{$n\_qubits$, $NK$, $idxs$, $coeffs$, $pmXY$, $pmYZ$, $batch\_size$, $batch\_size\_cur\_rank$, $ist$, $states$, $id\_lut$, $wf\_lut$}
\KwResult{$res\_elocs$}
\tcc{Initialization of power of two table}
$tbl\_pow2[0...63] \leftarrow \{1, 2,..., 2^{63}\}$ \;
\tcc{Partition for CUDA kernel}
$index \leftarrow blockIdx.x \times blockDim.x + threadIdx.x$ \;
$stride \leftarrow gridDim.x \times blockDim.x$ \;

\For{$ii \leftarrow index$ \KwTo $batch\_size\_cur\_rank$ \textbf{step} $stride$}{
    $eloc\_real, eloc\_imag \leftarrow 0$ \;
    \For{$k \leftarrow 0$ \KwTo $NK$}{
        \tcc{Fuse coupled states and state2id}
        $id \leftarrow 0$ \;
        \For{$j \leftarrow 0$ \KwTo $N$}{
            $id += xor(states[ii \times N+j], pmXY[k \times N+j]) \times tbl\_pow2[j]$ \;
        }
        \tcc{Binary find id among the lookup table}
        $idx \leftarrow binary\_find(id\_lut, id)$ \;
        \If{$idx$ \textbf{does not exist}}{
            \textbf{continue} \;
        }
        \tcc{Calculate coupled coef}
        $coef \leftarrow 0.0$ \;
        \For{$i \leftarrow idxs[k]$ \KwTo $idxs[k+1]$}{
            $sum \leftarrow 0$ \;
            \For{$j \leftarrow 0$ \KwTo $N$}{
                $sum += states[ii \times N+j] \& pmYZ[i \times N+j]$ \;
            }
            $coef += ( (sum \& 1) ? 1 : -1) \times coeffs[i]$ \;
        }
        \tcc{Accumulation}
        $eloc\_real += coef \times wf\_lut[idx \times 2]$ \;
        $eloc\_imag += coef \times wf\_lut[idx \times 2+1]$ \;
    }
    \tcc{Store the result number as return}
    $a, b \leftarrow eloc\_real, eloc\_imag$ \;
    $c, d \leftarrow wf\_lut[(ist+ii) \times 2], wf\_lut[(ist+ii) \times 2+1]$ \;
    $c2\_d2 \leftarrow c^2 + d^2$ \;
    $res\_elocs[ii \times 2] \leftarrow (a \times c + b \times d) / c2\_d2$ \;
    $res\_elocs[ii \times 2+1] \leftarrow -(a \times d - b \times c) / c2\_d2$ \;
}
\caption{Optimizations of local energy calculation}
\end{algorithm}

